GPT4Scene: Understand 3D Scenes from Videos with Vision-Language Models

In recent years, 2D Vision-Language Models (VLMs) have made significant strides in image-text understanding tasks. However, their performance in 3D spatial comprehension, which is critical for embodied intelligence, remains limited. Recent advances have leveraged 3D point clouds and multi-view images as inputs, yielding promising results. However, we propose exploring a purely vision-based solution inspired by human perception, which merely relies on visual cues for 3D spatial understanding. This paper empirically investigates the limitations of VLMs in 3D spatial knowledge, revealing that their primary shortcoming lies in the lack of global-local correspondence between the scene and individual frames. To address this, we introduce GPT4Scene, a novel visual prompting paradigm in VLM training and inference that helps build the global-local relationship, significantly improving the 3D spatial understanding of indoor scenes. Specifically, GPT4Scene constructs a Bird's Eye View (BEV) image from the video and marks consistent object IDs across both frames and the BEV image. The model then inputs the concatenated BEV image and video frames with markers. In zero-shot evaluations, GPT4Scene improves performance over closed-source VLMs like GPT-4o. Additionally, we prepare a processed video dataset consisting of 165K text annotation to fine-tune open-source VLMs, achieving state-of-the-art performance on all 3D understanding tasks. Surprisingly, after training with the GPT4Scene paradigm, VLMs consistently improve during inference, even without object marker prompting and BEV image as explicit correspondence. It demonstrates that the proposed paradigm helps VLMs develop an intrinsic ability to understand 3D scenes, which paves the way for a seamless approach to extending pre-trained VLMs for 3D scene understanding.

==> sup/tab/tab_gpt4o.tex <==
\begin{tabular}{lccccccc| cc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{\makecell[c] {Point \\ Encoder}} & \multirow{2}{*}{\makecell[c] {Vision \\ Encoder}}& \multicolumn{5}{c}{\textbf{ScanQA (val)}} & \multicolumn{2}{c}{\textbf{SQA3D (val)}}
\\\cmidrule(lr){4-8}\cmidrule(lr){9-10}
& &  & BLEU-1 & BLEU-4 & METEOR & ROUGE & CIDEr & EM-1 & EM-R1 
\\
\midrule
\multicolumn{5}{l}{\textit{Vision based Model \quad (Close-Source)}} \vspace{1mm} \\
\rowcolor{gray!15} GPT-4o &  &  & 30.9 & 10.6 & 15.2 & 32.6 & 66.0 & 40.3 & 46.1 \\
\rowcolor{gray!15} GPT-4o (GPT4Scene) &  &  & 35.6$\,_\text{\textcolor{darkgray}{+4.7}}$ & 12.5$\,_\text{\textcolor{darkgray}{+2.1}}$ & 15.6$\,_\text{\textcolor{darkgray}{+0.4}}$ & 37.7$\,_\text{\textcolor{darkgray}{+5.1}}$ & 73.5$\,_\text{\textcolor{darkgray}{+7.5}}$ & 42.8$\,_\text{\textcolor{darkgray}{+2.5}}$ & 49.4$\,_\text{\textcolor{darkgray}{+3.3}}$ \\
\midrule
\multicolumn{5}{l}{\textit{Vision based Model \quad (Open-Source)}} \vspace{1mm} \\

InternVL2-8B~\cite{InternVL} & \textcolor{Red}{\ding{55}} & \textcolor{Green}{\ding{51}} & 23.9 & 3.3 & 14.5 & 34.3 & 62.5 & 33.0 & 45.3 \\
MiniCPM-V-2.6~\cite{MiniCPM-V} & \textcolor{Red}{\ding{55}} & \textcolor{Green}{\ding{51}} & 25.1 & 8.4 & 11.8 & 31.5 & 60.1 & 42.6 & 46.6 \\
\rowcolor{green!7} Qwen2-VL-7B~\cite{Qwen2VL}  & \textcolor{Red}{\ding{55}} & \textcolor{Green}{\ding{51}} & 27.8 & 3.0 & 11.4 & 29.3 & 53.9 & 40.7 & 46.7 \\
\rowcolor{green!10} Qwen2-VL-7B (GPT4Scene) & \textcolor{Red}{\ding{55}} & \textcolor{Green}{\ding{51}} & {\textbf{43.4}$\,_\text{\textcolor{darkgray}{+15.6}}$} & {\textbf{14.6}$\,_\text{\textcolor{darkgray}{+11.6}}$} & 17.7$\,_\text{\textcolor{darkgray}{+6.3}}$ & {\textbf{43.6}}$\,_\text{\textcolor{darkgray}{+14.2}}$ & {\textbf{90.9}}$\,_\text{\textcolor{darkgray}{+37.0}}$ & {\textbf{57.4}}$\,_\text{\textcolor{darkgray}{+16.7}}$ & {\textbf{60.7}}$\,_\text{\textcolor{darkgray}{+14.1}}$ \\
\bottomrule
\end{tabular}


==> tab/tab_3d_dc_vg.tex <==
\begin{table*}[!t]
\begin{subtable}{\linewidth}
\centering
\setlength\tabcolsep{6pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l cccc|ccc|ccc}
\toprule
& \multicolumn{4}{c}{\textbf{Scan2Cap} (\textit{3D Dense Caption})} & \multicolumn{3}{c}{\textbf{ScanRefer} (\textit{3D Grounding})} & \multicolumn{3}{c}{\textbf{Multi3DRefer} (\textit{3D Grounding})}
\\\cmidrule(lr){2-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
\textbf{Model} & CIDEr & BLEU-4 & METEOR & ROUGE & CIDEr & CIDEr & CIDEr & CIDEr & ROUGE & CIDEr
\\
3D-LLM~\cite{3dllm} (\textit{for ref.}) & - & - & - & - & - & - & - & - & - & -\\
\midrule
DINOv2              & - & - & - & - & - & - & - & - & - & -\\
LSeg                & - & - & - & - & - & - & - & - & - & -\\
CLIP                & - & - & - & - & - & - & - & - & - & -\\

\bottomrule
\end{tabular}
}
\end{subtable}
\vspace{-2mm}
% \captionsetup{font=footnotesize}
\caption{\textbf{Evaluation of vision-language reasoning on ScanQA~\cite{scanqa} and SQA3D~\cite{sqa3d} datasets.} Top-2 results for each metric are shown in.}
\label{tab:scanqa}
\vspace{-4mm}  
\end{table*}


==> tab/tab_closed_source.tex <==
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Ablation} & \multicolumn{2}{c}{ScanQA} & \multicolumn{2}{c}{Multi3DRef@0.5} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& ROUGE & CIDEr & MT & ALL \\
\midrule
Qwen2-VL-7B (GPT4Scene) & 43.6 & 90.9 & 36.3  & 42.1 \\
w/o BEV Image  & 42.3 & 87.1 & 27.8  & 32.1 \\
w/o BEV Image \& STO markers & 41.7 & 85.0 & - & - \\

\bottomrule
\end{tabular}

